A Finite-Time Cutting Plane Algorithm for Distributed Mixed Integer Linear Programming

Many problems of interest for cyber-physical network systems can be formulated as Mixed Integer Linear Programs in which the constraints are distributed among the agents. In this paper we propose a distributed algorithm to solve this class of optimization problems in a peer-to-peer network with no coordinator and with limited computation and communication capabilities. In the proposed algorithm, at each communication round, agents solve locally a small LP, generate suitable cutting planes, namely intersection cuts and cost-based cuts, and communicate a fixed number of active constraints, i.e., a candidate optimal basis. We prove that, if the cost is integer, the algorithm converges to the lexicographically minimal optimal solution in a finite number of communication rounds. Finally, through numerical computations, we analyze the algorithm convergence as a function of the network size.

==> 100ag9croundp0015_64_zoomin.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%
%
\begin{tikzpicture}

\begin{axis}[%
width=3cm,
height=1.953cm,
at={(0cm,0cm)},
scale only axis,
xmin=3.61383807029834,
xmax=9.03465833521962,
%xlabel style={font=\bfseries\color{white!15!black}},
%xlabel={communication rounds},
ymin=-2.05373619945782,
ymax=4.04460594052106,
%ylabel style={font=\bfseries\color{white!15!black}},
%ylabel={$c^T z^{[i]}(t) - c^T z^*$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.47793712078301	4.65444015451895\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.07175604380621	3.78473186858137\\
4	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.85648791238758\\
4	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2.85648791238758\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.46911196909621	4.65444015451895\\
4	2\\
5	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
4	1\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2.92824395619379\\
4	2\\
5	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
4	1\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.95314820314719	4.65444015451895\\
4	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
4.39092664091351	4.65444015451895\\
5	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.85648791238758\\
4	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	0.928243956193791\\
4	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	3.78473186858137\\
4	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
4	1\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.47793712078301	4.65444015451895\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.54319498068513	4.65444015451895\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.70506220505345	4.65444015451895\\
4	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.99551753318823	4.65444015451894\\
4	4\\
5	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.54319498068513	4.65444015451895\\
4	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.39092664091351	4.65444015451895\\
4	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.07175604380621	3\\
4	3\\
5	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
4.95314820314719	4.65444015451895\\
5	1\\
8	1\\
9	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.85648791238758\\
4	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.96364221363784	4.65444015451894\\
4	4\\
5	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
5	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
5	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.54319498068513	4.65444015451895\\
4	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.97263463758228	4.65444015451895\\
4	2\\
5	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	3.85648791238758\\
4	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2.85648791238758\\
4	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.39092664091351	4.65444015451895\\
4	1\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.85648791238758\\
4	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2.92824395619379\\
5	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.55759330758018	4.65444015451895\\
4	2\\
5	2\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2.85648791238758\\
4	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
5.77879665379009	4.65444015451894\\
6	2\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
4.47793712078301	4.65444015451895\\
5	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
4	1\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
5	2\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
4	1\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
4	1\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
4.77879665379009	4.65444015451894\\
5	2\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.39092664091351	4.65444015451895\\
4	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
4	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.77879665379009	4.65444015451894\\
4	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	3\\
4	3\\
5	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2.92824395619379\\
5	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
6	1\\
7	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
4	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1.92824395619379\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
3.07175604380621	1\\
4	1\\
5	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
3.39092664091351	4.65444015451895\\
4	1\\
5	1\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
3.07175604380621	2\\
5	2\\
6	0\\
9.57674036171175	0\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
3.07175604380621	3.78473186858137\\
4	1\\
7	1\\
8	0\\
9.57674036171175	0\\
};
\end{axis}
\end{tikzpicture}%
